Taking a turn for the better: Conversation redirection throughout the course of mental-health therapy

Mental-health therapy involves a complex conversation flow in which patients and therapists continuously negotiate what should be talked about next. For example, therapists might try to shift the conversation's direction to keep the therapeutic process on track and avoid stagnation, or patients might push the discussion towards issues they want to focus on. How do such patient and therapist redirections relate to the development and quality of their relationship? To answer this question, we introduce a probabilistic measure of the extent to which a certain utterance immediately redirects the flow of the conversation, accounting for both the intention and the actual realization of such a change. We apply this new measure to characterize the development of patient-therapist relationships over multiple sessions in a very large, widely-used online therapy platform. Our analysis reveals that (1) patient control of the conversation's direction generally increases relative to that of the therapist as their relationship progresses; and (2) patients who have less control in the first few sessions are significantly more likely to eventually express dissatisfaction with their therapist and terminate the relationship.

==> 030data-anon.tex <==

\xhdr{Long-term text-based therapy}
We develop our methodology in the context of Talkspace,
a telehealth 
therapy
platform.
Patients can choose between different plans, which may include video 
therapy alongside messaging therapy. 
After a consultation in which they answer a few questions about their symptoms and describe their preferences, patients are matched by the platform to a suitable therapist who is licensed in their state.

In this work, we use the (English-language) text-based 
conversations
(after redaction of personally identifiable information by Talkspace) from a five-year span.\footnote{The use of the therapist and patient data is done with their consent, and this research was approved by the 
appropriate institutional IRB.}
During this time, Talkspace hosted over 18,000 licensed therapists providing services to over 300,000 patients.
In total, over 65 million 
messages were exchanged.

Therapies can be sustained over long periods of time, with 
more than 26,000 therapies lasting over a year and 17,000 therapies comprising over 500 messages.
This setting thus provides an opportunity to study the long-term conversational
dynamics as the therapeutic relationship develops.

At any point, patients can either cancel their therapy or switch to a different therapist.  
When doing so, they are asked to provide a reason, either by selecting from a drop-down menu (e.g., ``The treatment provided by my therapist was not helpful,'' ``I met my goal / I feel better'') or by entering free text.
We have some assurance that these reasons are authentic because patients are informed that therapists cannot access them.
These reasons serve as imperfect indicators of the perceived quality of the therapeutic relation (for a broader discussion of difficulties in operationalizing the quality of the therapeutic 
relationship, see Section~\ref{sec:limitations}).

\xhdr{Session identification}
One challenge in studying the development of therapeutic relationships in this text-based setting is accounting for the wide variety of durations, tempos, and volubility exhibited in different therapies.
A longitudinal analysis requires a methodology that captures the progression of the therapeutic process while allowing for meaningful aggregation across therapies with these vastly different interaction patterns.

To address this challenge, we need to account for several factors.
First, each therapist-patient pair develops a unique interaction style and tempo, including frequency of interaction, response time, and how often turns are split into multiple messages.
Second, exchanges between a therapist and a patient include not only therapeutic conversation, but also short check-ins that deal with brief updates, scheduling, or survey completions.
Last, an important component of many therapies is the occurrence of spans of {\em approximately synchronous} conversations, or \textit{sessions}, over the therapy's duration.
These three factors render conventional units of progression in conversational analysis---such as time or number of utterances---unsuited for this complex interactional setting.

Explicit session boundaries are lacking in text-based conversations and so must be inferred.
We start by distinguishing high-activity periods interwoven with periods of little or no activity, using the method from \citet{kushner_bursts_2020} to capture these bursts.
For each therapy, we
define session-split points as moments when an utterance's reply time 
exceeds $N \times$ (\textit{median reply time of that entire therapy}).\footnote{
We settle on $N=100$; see Appendix \ref{sec:appendixsessionsplit} for details.}
We further ensure that each session represents an actual conversation between the patient and the therapist (as opposed to, for example, a short notification and acknowledgement regarding scheduling) 
by filtering out short exchanges---any burst of activity with fewer than four turns (so that what remains includes at least two nonconsecutive utterances from each speaker)---or includes a video session.
We further remove any automated messages related to video sessions, survey completion, or scheduling.

To validate the quality of the session splits,
we sampled therapies with at least 10 sessions and ran 
a Bayesian distinguishing-word analysis \cite{monroe_fightin_2017} on the first and last utterance of each session.
The distinguishing words are intuitive: sessions start with greetings ("hi", "morning", "hey", "how") and end with a farewell or expression of gratitude ("enjoy", "welcome", "thank", "thanks").



%

